Fundamental Physics at the Intensity Frontier

The Proceedings of the 2011 workshop on Fundamental Physics at the Intensity Frontier. Science opportunities at the intensity frontier are identified and described in the areas of heavy quarks, charged leptons, neutrinos, proton decay, new light weakly-coupled particles, and nucleons, nuclei, and atoms.

==> ProtonDecay/lbne.tex <==
LBNE is planning for two 
types of detectors at an underground site in Homestake, South Dakota: a 
200 kt water Cherenkov (WCh) detector or a 34 kt liquid Argon (LAr) TPC. 
These detectors have complementary strengths in the search for proton decay, 
and either represents a considerable step forward from existing 
facilities. (At the time of this writing the LAr option has 
been chosen for the LBNE far detector technology. However, in order 
to be complete the proton decay sensitivities of both detector options are 
described in this report.) 

\paragraph{Liquid Argon TPC:} 
This detector would be a significant size scale-up of the current largest 
liquid Argon TPCs, the 300~t ICARUS modules that came into full 
underground operation in 2010. The plan is for two separate 
modules, each of 16.5~kt fiducial mass. While this is less than a 
factor of two larger than Super-K (22 kt), the ability to observe 
charged particle tracks below the Cherenkov threshold in water means 
that some modes poorly observed in Super-K would be much better 
measured in LBNE LAr. For example, there is a significant 
sensitivity increase for the supersymmetric grand unified theories 
motivated mode $p \rightarrow \bar{\nu} K^+$.  
The charged kaon, with a momentum of 340 MeV/c (neglecting nuclear effects), 
has a range of 14~cm in LAr, so ionization energy loss measurements 
are expected to give high particle identification efficiency. 
The $K^+$ will also decay at rest to fully reconstructable final states 
such as a muon with reconstructed momentum of 236~MeV/$c$ and no other 
visible particle, a clear signature for 
$K^+ \rightarrow \mu^+\nu$ (65\% branching fraction). 
Therefore efficiency in excess of 90\% with very low background 
from atmospheric neutrinos is quite plausible. 
In contrast, since the $K^+$ has a relativistic gamma of 1.2, 
below the water Cherenkov threshold of 1.5, in Super-K 
this mode is measured only by the less-efficient gamma tag method. 
The LAr efficiency for this mode is roughly a factor of five higher than 
Super-K, as shown in Fig.~\ref{fig:LBNE_pdk_sensitivities}. 
The top curve in the left panel shows the sensitivity that could be 
reached assuming the full active volume can be used. 
Also shown are the expectations if only one module is built (dotted) or 
a significant fiducial volume cut is needed (dashed) to reduce cosmogenic 
backgrounds.  The most serious background is from neutral kaons 
produced by cosmic ray interactions in the surrounding rock that 
subsequently undergo charge exchange in the sensitive volume. 
These could result in the appearance of a charged kaon that mimics 
proton decay if the $K^+$ has the right momentum. This background 
process will be studied by measuring the rate of such events 
in momentum sidebands, but cutting out candidates near the side walls 
will eliminate such events at a cost of reduced fiducial mass. 
In the Bueno {\it et al.} paper~\cite{Bueno:2007um}, 
several different overburden and active veto scenarios were considered, 
with fiducial cuts as much as 7 meters from the wall, 
resulting in fiducial mass reductions ranging from 66\% to 90\%. 
A 2-meter cut from the sidewalls of the planned LBNE
detector, reduces the volume by 70\% from 
14$\times$15$\times$71~meters$^3$ to 14$\times$11$\times$67~meters$^3$, 
corresponding roughly to the dotted lines in 
Fig.~\ref{fig:LBNE_pdk_sensitivities}. 
The current LBNE reference design locates the LAr at the 4850-ft 
level of Homestake to mitigate this background; 
if the detector is located at the 800-ft level a substantial 
muon tracking veto system will also be required. 

The $p \rightarrow e^+ \pi^0$ mode can be detected in LAr 
with an expected efficiency somewhat lower than the 45\% efficiency 
achieved in WCh, which is set by the irreducible pion absorption rate 
in the nucleus. Although not yet calculated explicitly, 
the expected efficiency reduction should scale roughly with the 
linear size of the nucleus. Thus a naive estimate would be 
$45\% \times (16/39)^{1/3} = 33\%$. Even with a very low background 
rate of 0.1 events per 100~kt-years~\cite{Bueno:2007um}, 
the improvement in sensitivity compared to Super-K is not significant.
 
\paragraph{Water Cherenkov Detector:} The water Cherenkov detector 
planned is roughly nine times larger than Super-K, 
and hence for modes with no background sensitivity will simply 
scale with volume. For modes like $p \rightarrow e^+ \pi^0$ 
some amount of background is expected in the LBNE regime
based on measurements done by the K2K experiment, which also validated 
the neutrino simulations used for the water Cherenkov experiments. 
The level of expected background 
is 2 events/Mton/year, all from atmospheric neutrino interactions.
 
The right panel in Fig.~\ref{fig:LBNE_pdk_sensitivities} 
shows the sensitivity that could be reached in this mode 
assuming no background improvements are made (red line). 
In fact, it may be possible to significantly reduce this background 
if a neutron detection capability (such as addition of Gadolinium) 
is realized. This is due to the fact that while 80\% of proton decays 
in water should not have associated neutrons, atmospheric neutrino 
interactions are likely to produce one or more neutrons. 
These neutrons come from direct production via anti-neutrinos on oxygen, 
final state scattering of hadrons and $\pi^-$ capture on oxygen, 
and nuclear de-excitation. The figure shows the sensitivity reached 
if improvements allow rejection of all atmospheric neutrino backgrounds 
(blue line). The actual efficiency for background rejection will require 
measurements in a neutrino beam, and such an experiment is being 
planned for the FNAL booster neutrino beam.

\begin{figure}
  \begin{center}
    \includegraphics[width=0.49\textwidth]{ProtonDecay/figures/LBNE_pdk_lar_sensitivity.pdf}
    \includegraphics[width=0.49\textwidth]{ProtonDecay/figures/LBNE_pdk_wcd_sensitivity.pdf}
  \end{center}
  \caption{\label{fig:LBNE_pdk_sensitivities} 
  The LBNE projected sensitivities for proton decay searches as a function 
  of calendar year. 
Left panel: the sensitivity of the liquid argon detector option 
for the $p \rightarrow \bar{\nu} K^+$ mode; 
Right panel: the sensitivity of the water Cherenkov detector option
for the $p \rightarrow e^+ \pi^0$ mode. The dashed arrow marked as 
``WC 560'' is the expected sensitivity by Hyper-K around year 2040, 
assuming, of course, it will be built as proposed.}
\end{figure}


==> tcilcomm.tex <==
% Macros used for TCI styles released with Scientific Word 1.1.
%Copyright (C) 1992-93 TCI Software Research, Inc.
\typeout{TCILCOMM Macros for TCI styles <08 Apr 93>.}
%
% Revisions:
% 08 Apr 93 - GP change line length to under 80 characters
% 30 Mar 92 - AO added \setmoremathsizes and hooks to, e.g. \@xpt,
%             for support of bold Greek
%
%%ltg added this to try to get 12pt to come through
%\DeclareOption{12pt}{\renewcommand\@ptsize{2}}
%%end ltg

\def\@ptoptions{%
 \let\@elt\relax\@for\@tempa:=\@optionlist\do{%
  \expandafter\let\expandafter\@tempb\csname ds@\@tempa\endcsname
  \expandafter\let\expandafter\@tempc\csname ds@11pt\endcsname
  \ifx\@tempb\@tempc\else
   \expandafter\let\expandafter\@tempc\csname ds@12pt\endcsname
   \ifx\@tempb\@tempc\else\let\@tempb\relax\fi
   \fi
  \@tempb
  }%
 }%
%
% read in style file, but only process the pt size options
%
\def\@ptoptinput#1{%
 \let\@save@optionlist\@optionlist
 \let\@save@options\@options
 \let\@options\@ptoptions
 %
 \input #1
 %
 \let\@optionlist\@save@optionlist
 \let\@options\@save@options
 }%
%
% the <21 Feb 92> version of letter.sty requires:
\ifx\undefined\reset@font
 \def\reset@font{}%
 \fi
%
% Change LaTeX
%
% Add command to append tokens
\newtoks\@temptokenb
\long\def\appdef#1#2{%
 \ifx#1\undefined\let#1\@empty\fi
 \@temptokena\expandafter{#1}\@temptokenb{#2}%
 \edef#1{\the\@temptokena\the\@temptokenb}%
 }%
\long\def\prepdef#1#2{%
 \ifx#1\undefined\let#1\@empty\fi
 \@temptokena\expandafter{#1}\@temptokenb{#2}%
 \edef#1{\the\@temptokenb\the\@temptokena}%
 }%
% Discard contents of \box\@cclv at beginning of document
\appdef\document{{\output{\setbox\z@\box\@cclv}\endgraf\null\eject}}%
% Fix mark register expansion
\def\leftmark{\expandafter\@leftmark\botmark{}{}{}\@nil}%
\def\rightmark{\expandafter\@rightmark\firstmark{}{}{}\@nil}%
\def\@leftmark#1#2#3\@nil{#1}%
\def\@rightmark#1#2#3\@nil{#2}%
%
%\show\raggedright
\newskip\raggedglue
\raggedglue\z@ plus20\p@ minus\z@
\def\raggedright{%
 \let\\=\@centercr\@rightskip\raggedglue\rightskip
 \@rightskip\leftskip\z@\parindent\z@
 }%
%
\def\@centercr{%
 \ifhmode\unskip\else\@badcrerr\fi\@@par
 \@ifstar{\penalty\@M\@xcentercr}{\@xcentercr}%
 }%
%
\def\traceoutput{\tracingoutput2\showboxbreadth\maxdimen
 \showboxdepth\maxdimen}%
%
\newcount\@hour\newcount\@minute\chardef\@x10\chardef\@xv60
\def\@time{%
  \@minute\time\@hour\@minute\divide\@hour\@xv
  \ifnum\@hour<\@x 0\fi\the\@hour:%
  \multiply\@hour\@xv\advance\@minute-\@hour
  \ifnum\@minute<\@x 0\fi\the\@minute
  }%
%
% change \@array to allow \par to mean something within its scope
%
\def\@array [#1]#2{%
 \setbox\@arstrutbox\hbox{\vrule height\arraystretch\ht
  \strutbox depth\arraystretch\dp\strutbox width\z@}%
 \@mkpream{#2}%
 \edef\@preamble{\halign\noexpand\@halignto\bgroup\tabskip
  \z@\@arstrut\@preamble\tabskip\z@\cr}%
 \let\@startpbox\@@startpbox\let\@endpbox\@@endpbox
 \if#1t\vtop\else\if#1b\vbox\else\vcenter\fi\fi
 \bgroup
  %\let\par\relax
  \let\@sharp##
  \let\protect\relax
  \lineskip\z@\baselineskip\z@
  \@preamble
 }%
%
% Expands to hex digit corresponding to the value of the argument
%
\def\hexnumber@#1{\ifnum#1<10 \number#1\else
 \ifnum#1=10 A\else\ifnum#1=11 B\else\ifnum#1=12 C\else
 \ifnum#1=13 D\else\ifnum#1=14 E\else\ifnum#1=15 F\fi\fi\fi\fi\fi\fi\fi}%
%
% define command to set more math sizes.
% Styles like Greekbf will hook in here.
%
\def\setmoremathsizes#1#2#3{}%
%
% define size switch addenda
%  Note: these choices agree with those in lfonts.tex, even if incorrect.
%
\prepdef\@vpt{\setmoremathsizes{fiv}{fiv}{fiv}}%
\prepdef\@vipt{\setmoremathsizes{six}{six}{six}}%
\prepdef\@viipt{\setmoremathsizes{sev}{fiv}{fiv}}%
\prepdef\@viiipt{\setmoremathsizes{egt}{six}{fiv}}%
\prepdef\@ixpt{\setmoremathsizes{nin}{six}{fiv}}%
\prepdef\@xpt{\setmoremathsizes{ten}{sev}{fiv}}%
\prepdef\@xipt{\setmoremathsizes{elv}{egt}{six}}%
\prepdef\@xiipt{\setmoremathsizes{twl}{egt}{six}}%
\prepdef\@xivpt{\setmoremathsizes{frtn}{ten}{sev}}%
\prepdef\@xviipt{\setmoremathsizes{svtn}{twl}{ten}}%
\prepdef\@xxpt{\setmoremathsizes{twty}{frtn}{twl}}%
\prepdef\@xxvpt{\setmoremathsizes{twty}{twty}{svtn}}%
%
% The \newfield command defines (like \newenvironment) a user syntax:
%
%   \newfield{foo}
%
% lets you write
%
%   \begin{foo}...\end{foo}
%
% but differs from \newenvironment in that TeX parses the entire content
% of the field and stores it in a macro \the@foo, and then executes \@do@foo.
%
% This means that the content of the field is actually more like an argument
% than the content of an environment. So \verb will not necessarily work
% within a field, and neither will \index. Caveat emptor.
%
% The default procedure for a field is to process its argument within a
% group.  If you want a field to simply store its data away, define its
% procedure to be synonymous with \@empty, as illustrated below.
%
\long\def\@readenvir#1#2\end{%
 \appdef\envirsofar{#2}%
 \@ifnextchar\bgroup{\@checkenvir{#1}}{\@envirenderr}%
 }%
%
\def\@envirenderr{%
 \@latexerr{\string\end\space not followed by environment name}\@eha
 }%
%
\def\@checkenvir#1#2{%
 \def\@tempa{#1}\def\@tempb{#2}%
 \ifx\@tempa\@tempb
  \ifx\envirsofar\@blankspace\let\envirsofar\@empty\fi
  \expandafter\let\csname the@#1\endcsname\envirsofar
  \def\@tempa{\csname @do@#1\endcsname}%
  \else
  \appdef\envirsofar{\end{#2}}%
  \def\@tempa{\@readenvir{#1}}%
  \fi
 \@tempa
 }%
%
\def\newfield#1#2{%
 \expandafter\@ifdefinable\csname#1\endcsname{%
  \expandafter\def\csname#1\endcsname{%
   \endgroup\let\envirsofar\@empty\@readenvir{#1}%
   }%
  \expandafter\let\csname the@#1\endcsname\@empty
  \expandafter\ifx\csname @do@#1\endcsname\relax
   \expandafter\def\csname @do@#1\endcsname{{\csname the@#1\endcsname}}%
   \fi
  }%
 }%
%
\def\@blankspace{ }% SciWord's nil field
%
\def\letparBL{\def\par{\\}}%
\def\letparSP{\def\par{\ }}%
\def\letparQD{\def\par{\quad}}%
\def\letparSL{\def\par{\hbox to1em{\hfil/\hfil}}}%
%
% When \par is processed in the page head, gobble up the rest of the
% argument.
\def\@gobblepar#1\@empty{}%
%
% Physical page size after trim
\newdimen\trimwidth
\newdimen\trimheight
\newdimen\botmargin
\newdimen\marginpartotal
%
\def\adjustpagemargin{% adjust \oddsidemargin by \marginpartotal
 \marginpartotal\marginparwidth\advance\marginpartotal\marginparsep
 \advance\oddsidemargin\marginpartotal
 }%
%
\def\settextheight{% calculate textheight constrained by:
 \textheight\trimheight
 \advance\textheight-\topmargin
 \advance\textheight-\headheight
 \advance\textheight-\headsep
 \advance\textheight-\footskip
 \advance\textheight-\botmargin
 }%
%
\def\vcenterpagemargin{% calculate \topmargin constrained by:
 \topmargin\trimheight
 \advance\topmargin-\textheight
 \advance\topmargin-\headheight
 \advance\topmargin-\headsep
 \advance\topmargin-\footskip
 \divide\topmargin\tw@\botmargin\topmargin
 }%
%
\def\centerpagemargin{% calculate \oddsidemargin constrained by:
 \oddsidemargin\trimwidth
 \advance\oddsidemargin-\textwidth
 \advance\oddsidemargin-\marginparwidth
 \advance\oddsidemargin-\marginparsep
 \divide\oddsidemargin\tw@
 \evensidemargin\oddsidemargin
 \adjustpagemargin
 }%
%
\def\leftpagemargin{% calculate \oddsidemargin constrained by:
 \oddsidemargin\trimwidth
 \advance\oddsidemargin-\textwidth
 \advance\oddsidemargin-\marginparwidth
 \advance\oddsidemargin-\marginparsep
 \advance\oddsidemargin-\evensidemargin
 \adjustpagemargin
 }%

